Deterring Searches for Child Sexual Abuse Material on Google Search and Promoting Help-Seeking

Google Search deploys a "Onebox" feature at the top of the results page when users conduct searches for Child Sexual Abuse Material. This study evaluates the impact of a strategic shift in this feature, comparing a revised intervention, focused on repercussions and therapeutic resources, to a previous iteration that focused on reporting. Using a difference-in-differences analysis of internal Google Search logs data, we found the new messaging resulted in a 3.8 percentage point reduction as compared to the status quo in subsequent CSAM-related queries within the same Search session. We found an average click through rate of 0.73% on any of the hyperlinked buttons to help-providing resources. Together, this research presents convergent evidence that a subset of individuals can be deterred from ongoing CSAM-seeking and redirected to therapeutic services.

==> master/robustness.tex <==
\begin{table}[ht]
\centering
\caption{Countries and languages included in Robustness check}
\begin{tabular}{lrr}
  \hline
  Country & Treated Language(s) & Untreated Language(s)\\ 
  \hline
  Australia & English & Chinese\\ 
    Belgium & Dutch, French & English \\ 
    Canada & English & Arabic, Persian \\ 
    France & French & Arabic, English \\ 
    Germany & German & Arabic, English, Persian, Russian \\ 
 
    Netherlands & Dutch & English, Russian\\ 
    United States & English & Spanish\\ 
   \hline
\end{tabular}
\label{robustness}
\end{table}
